Unsupervised ANN-Based Equalizer and Its Trainable FPGA Implementation

In recent years, communication engineers put strong emphasis on artificial neural network (ANN)-based algorithms with the aim of increasing the flexibility and autonomy of the system and its components. In this context, unsupervised training is of special interest as it enables adaptation without the overhead of transmitting pilot symbols. In this work, we present a novel ANN-based, unsupervised equalizer and its trainable field programmable gate array (FPGA) implementation. We demonstrate that our custom loss function allows the ANN to adapt for varying channel conditions, approaching the performance of a supervised baseline. Furthermore, as a first step towards a practical communication system, we design an efficient FPGA implementation of our proposed algorithm, which achieves a throughput in the order of Gbit/s, outperforming a high-performance GPU by a large margin.

==> chapters/channel_model.tex <==
\begin{figure}[tbp]
	\centerline{\input{figures/tikz_channel.tex}}
	\caption{Generalized channel model where the vector $\bm{x}$ contains the transmitted symbols, $\bm{h}_{\mathrm{ps}}$ and $\bm{h}_{\mathrm{ch}}$ are the linear impulse responses of the pulse shaping filter and the channel, $f_{\mathrm{rx}}$ describes a potential non-linear distortion (which is applied element-wise), $\bm{n}$ is \ac{awgn}, and $\bm{y}$ is the received vector.}
	\label{fig:channel}
\end{figure}

We demonstrate the flexibility of our approach by evaluating it under different, both linear and nonlinear, communication channels. All simulated channels can be described by the generalized model in Fig.~\ref{fig:channel}, where the transmitted symbols, represented by the vector $\bm{x}$, are convolved with a \ac{rc} pulse shaping filter $\bm{h}_\mathrm{ps}$ (with roll-off $\rho_\mathrm{rc}=0.25$) and a linear channel impulse response $\bm{h}_\mathrm{ch}$. Specific receiver characteristics can be described by a function $f_\mathrm{rx}\mlr{\cdot}$, which is element-wise applied to a vector. Finally, the received vector $\bm{y}$ is superimposed by a Gaussian noise vector $\bm{n}$. Since oversampling is essential to real systems, we run all simulations at an oversampling rate of $\Nos=2$~\ac{sps}.

% Precisely, we simulate linear telephone channels as described in \cite[Ch.~9.4-3]{proakis2008digital}, known as \emph{Proakis-A} (ProA) and \emph{Proakis-B} (ProB), with equivalent discrete-time impulse responses
% \begin{align*}
% 	\bm{h}_{\mathrm{ch,\, ProA}} &= [0.04, \ -0.05, \ 0.07, \	-0.21, \ -0.5, \ 0.72,\\
% 	&\hspace*{30mm} 0.36, \ 0, \ 0.21, \ 0.03, \ 0.07] \\
% 	\bm{h}_{\mathrm{ch,\, ProB}} &= [0.407, \ 0.815, \ 0.407] \; .
% \end{align*}
% In this case, we use real-valued \ac{bpsk} and 4-ary \ac{ask} for modulation and have $f_\mathrm{rx}\mlr{\tilde{\bm{x}}}=\tilde{\bm{x}}$.
Precisely, we simulate the bad-quality linear telephone channel described in \cite[Ch.~9.4-3]{proakis2008digital}, known as \emph{Proakis-B} (ProB), with equivalent discrete-time impulse response
\begin{align*}
	\bm{h}_{\mathrm{ch,\, ProB}} &= [0.407, \ 0.815, \ 0.407] \; ,
\end{align*}
which we upsample to $\Nos=2$~\ac{sps} by interleaving a zero between each tap. The pulse shaping filter then interpolates both the channel and the transmitted vector (which is also upsampled by inlerleaving zeros). 
For the linear channel, we use a real-valued \ac{bpsk} modulation and have $f_\mathrm{rx}\mlr{\tilde{\bm{x}}}=\tilde{\bm{x}}$. 

%\begin{table}[b!]
%	\caption{Characteristics of an \ac{ssmf}}\label{tab:ssmf_parameters}
%	\centering
%	\begin{tabular}{lll}
%		\hline
%		\textbf{Parameter}      &       & \textbf{Value} 	\\ \hline\hline
%		Wavelength & & $\lambda = \SIrange{1530}{1565}{\nano\meter}$ (C-Band) 	\\ 
%		Chromatic dispersion & & $D = \SI{17}{\CD}$ 		\\ 
%		Attenuation & & $\alpha_{\text{dB}} = \SI{0.2}{\FL}$ 	\\
%		\hline
%		%\vspace{0.1cm}
%	\end{tabular}
%\end{table}

Additionally, we simulate a nonlinear, dispersive optical channel with \ac{imdd} and \ac{pam} as described in \cite{plabst_wiener}. The \ac{sld} at the receiver distorts the signal nonlinearly and can be modeled by
$\tilde{\bm{y}} = f_\mathrm{rx}\mlr{\tilde{\bm{x}}}$ with $\tilde{y}_i=|\tilde{x}_i|^2$. % $f_\mathrm{rx}\mlr{\tilde{\bm{x}}}=|\tilde{\bm{x}}|^2$ (i.e., the vector's absolute-square)
Linear channel distortions are caused by \ac{cd}, which can be described (including attenuation) by its frequency response
\begin{equation*}
	H_\mathrm{cd}\left( \Lf, f \right) = \exp\left(- \frac{1}{2} \alpha \Lf \, + \, \j 2 \pi^2 \beta_2 f^2 \Lf\right)  \label{eq:cd_freqency_response}
\end{equation*}
where $\Lf$ is the fiber length, $\beta_2=-\frac{\lambda^2}{2\pi \mathrm{c}} D_\mathrm{cd}$ is defined by the wavelength $\lambda$, the speed of light $\mathrm{c}$ and the fiber's dispersion coefficient $D_\mathrm{cd}$; and $\alpha$ is the fiber attenuation.
This work considers  C-band transmission at $\lambda=\SI{1550}{\nano\meter}$ over a \ac{ssmf}, i.e., $D_\mathrm{cd} = \SI{17}{\CD}$ and $\alpha \triangleq \SI{0.2}{\FL}$.

As both the pulse shaping filter and \ac{cd} filter are linear and time-invariant, we can define the \acl*{cir} 
\begin{equation*}
    \bm{h}_\text{cir} = \bm{h}_\text{ps}\ast \bm{h}_\text{ch} = \mathcal{F}^{-1}\mlrb{\bm{H}_\text{ps}\cdot \bm{H}_\text{cd}} 
\end{equation*}
where $\mathcal{F}^{-1}\mlrb{\cdot}$ is the inverse Fourier transform and $\bm{H}_\text{ps}$ is the frequency response of the pulse shaping filter. 

Following \cite{plabst_wiener},~\cite[ch.~4]{Agr10}, we assume to have no optical amplifiers, so the dominant noise source is the thermal noise in the electronic domain after the \ac{sld}, which can be modeled as \ac{awgn} with zero-mean and the variance $\varN$. For the simulation, we fix the \ac{snr} to $\SI{20}{dB}$ (PAM-2) and $\SI{26}{dB}$ (PAM-4). 
At the receiver, we conduct hard decision based on the minimum Euclidean distance and compensate for shifts, scaling-offsets, inversions and permutations, which can occur at blind equalization. In real systems, this can be done by transmitting a header or testing the possible combinations with the \ac{fec} decoder.

%Then, the overall input-output relation can be expressed as
%\begin{align}
%    \bm{y} = \lr{\bm{x} \ast \bm{h}_\text{cir}}^2 + \bm{n} \; .
%\end{align}
% 
%Auf Ebene der pdf/pmf einführen --> dann Übergang zu GAN über pmf lernen?

% \Cref{fig:gan_approach} depicts an overview of the approach. We use a discrete model to simulate the \ac{imdd} communication system as described in \cite{plabst_wiener}. The model employs a raised-cosine transmit filter $h_\text{tx}$, and ideal receive filter (which can be omitted for oversampling rate of 2 \ac{sps} \cite{plabst_wiener}) to avoid \ac{isi} from pulse-shaping. Effectively, the \ac{imdd} system affects the transmit symbols by a linear \ac{cd} filter and subsequent \ac{sld}. In literature the \ac{cd} filter is commonly described in frequency domain, which leads to the following frequency response for a lossy fiber of length $L_\text{fiber}$
% \begin{equation}
% 	H_\text{cd}\left( L_\text{fiber}, f \right) = \exp\left(- \frac{1}{2} \alpha_\text{dB} L_\text{fiber} \, + \, \text{j} 2 \pi^2 \beta_2 f^2 L_\text{fiber}\right) \; , \label{eq:cd_freqency_response_1}
% \end{equation}
% with group velocity delay $\beta_2$ and fiber attenuation $\alpha_\text{dB}$.
% \Ac{cd} is characterized by the parameter 
% \begin{equation}
%     D = \frac{d}{d \lambda}\left(\frac{1}{v_\text{g}}\right) = -\frac{2\pi\text{c}}{\lambda^2} \beta_2
% \end{equation}
% for wavelength $ \lambda $ and speed of light $ \text{c} $. \Cref{tab:ssmf_parameters_1} summarizes the parameters of a \ac{ssmf}, which is considered in this work.

% \begin{table}
% 	\centering
% 	\begin{tabular}{lll}
% 		\hline
% 		\textbf{Parameter}      &       & \textbf{Value} 	\\ \hline\hline
% 		Wavelength & & $\lambda = \SIrange{1530}{1565}{\nano\meter}$ (C-Band) 	\\ 
% 		Chromatic dispersion & & $D = \SI{17}{\CD}$ 		\\ 
% 		Attenuation & & $\alpha_{\text{dB}} = \SI{0.2}{\FL}$ 	\\
% 		\hline
% 		\vspace{0.1cm}
% 	\end{tabular}
% 	\caption{Characteristics of an \ac{ssmf}.}
% 	\label{tab:ssmf_parameters_1}
% \end{table}

% The frequency response $H_\text{cd}\left( L_\text{fiber}, f \right)$ \eqref{eq:cd_freqency_response} is sampled and inverse Fourier-transformed to obtain a discrete representation of the channel impulse response $h_\text{cd}[k]$. As both systems, the transmit filter and \ac{cd}-filter are modelled as linear time-invariant systems, their \ac{cir} $h_\text{cir}[k]$ is given by
% \begin{equation}
%     h_\text{cir}[k] = (h_\text{tx}*h_\text{cd})[k] = \sum_{m=-\infty}^{\infty} h_\text{tx}[m] h_\text{cd}[k-m] \; .
% \end{equation}
% The \ac{cir} $h_\text{cir}[k]$ is computed in advance for an oversampling rate of 2 \ac{sps} and applied in a single convolution operation during simulation.

% Following \cite{plabst_wiener,Agr10}, thermal noise in the \ac{sld} at the receiver is considered as dominant noise source. We incorporate these imperfections as additive white Gaussian noise with noise power $\sigma_n^2$ and discrete realizations $n$ at the output of the \ac{sld}.



==> chapters/hardware_architecture.tex <==
\section{Hardware Architecture}
\label{sec:hardware_architecture}

A major constraint for high-performance hardware implementation of \acp{ann} is the restricted on-chip memory of the \ac{fpga}. The efficient quantization presented in Sec.~\ref{Sec:quantization} is a first step to reduce the memory footprint. However, in contrast to most previous works, we also implement the training of the \ac{ann} on the \ac{fpga}, which requires additional resources. To perform backpropagation, a large amount of memory is required to store the feature maps of the \ac{fp} to be reused in the \ac{bp}. For high sequence lengths, the \ac{fpga}'s on-chip memory is usually not sufficient to store those feature maps, thus offloading to external DRAM is necessary, resulting in limited throughput. For instance, storing a sequence with the length of one Ethernet frame (\SI{1518}{byte}) requires four times as many \acp{bram} as utilized by the whole remaining architecture. Moreover, storing \num{5} Ethernet frames on-chip even exceeds the available \ac{bram} of a high-end \ac{fpga} like the \textit{Xilinx XCZU9EG\nobreakdash-2FFVB1156}.\\
To solve this problem, we propose a fully pipelined architecture in which we balance the lifetime of the feature maps such that the memory footprint is reduced, as sketched in Fig.~\ref{fig:hardware_architecture}. 

\begin{figure}[b]
	\centerline{\input{figures/tikz_hardware_architecture.tex}}
	\caption{Hardware architecture of trainable with kernel size $K$, padding $P$, stride $S$, dilation $D$ and number of channels $N_{ch}$. Arrows indicate streams of feature maps, either between subsequent layers or between \ac{fp} and \ac{bp}. Feature map buffers are shown in red.
 }
	\label{fig:hardware_architecture}
\end{figure}


\begingroup
\abovedisplayskip=8pt 
\belowdisplayskip=8pt

In our hardware architecture, all modules of \ac{fp} (shown in green) and \ac{bp} (shown in blue) are implemented as separate pipeline stages. The forward blocks (Conv) calculate the channel-wise discrete convolution of input $i$ with kernel $k$ and apply the \ac{relu} activation function
\begin{equation}
\label{eq_1}
%o_n = \max(\sum_{i = -\lfloor \frac{K}{2} \rfloor}^{\lfloor \frac{K}{2} \rfloor} x_{n-i} \cdot k_i, 0) \quad \forall n \in N
o = \mathrm{ReLU}(i \ast k) \; .
\end{equation}
The backward blocks (CalcGrad) consist of two modules: one to calculate the input's gradient (CalcInGrad) and another one to calculate the kernel's gradient (CalcKGrad). The input's gradient $\nabla i$ is given as the channel-wise convolution of the flipped kernel with the output gradient $\nabla o$:
\begin{equation}
\label{eq_2}
\nabla i = \mathrm{flip}(k) \ast \nabla o \; ,
\end{equation}
while the kernel gradient $\nabla k$ can be obtained by convolving the input with the output gradient:
\begin{equation}
\label{eq_3}
\nabla k = i \ast \nabla o \; .
\end{equation}
\endgroup


The core of our hardware architecture is a highly customizable convolutional module, which allows for variable kernel size, padding, stride, and dilation. Each convolution of the \ac{cnn} is implemented as a separate hardware module, enabling parallel computation of each layer and therefore increasing the overall throughput, which is crucial for high-performance communication systems. Since filling and flushing the pipeline is neglectable for high sequence lengths, the overall throughput is approximately the same as the minimum throughput of all layers.

To solve the problem of large feature map buffers between the \ac{fp} and \ac{bp}, we take advantage of the sequential nature of convolution operations \eqref{eq_2} and \eqref{eq_3} in the \ac{bp}. The calculation of $\nabla i$ and $\nabla k$ can already start before all elements of $i$ and $\nabla o$ are available. Since \ac{fp} and \ac{bp} are implemented as separate pipeline stages, they can be processed in parallel. Therefore, the feature maps are read and written concurrently and the size of the buffers can be greatly reduced.
Moreover, we designed our layers in a way that \ac{fp} and \ac{bp} have similar latency. Hence, the size of the feature map buffers is determined only by the depth of the pipeline and does not depend on the length of the sequence. This enables processing symbol sequences of arbitrary length. Thus our approach is suited for many different application scenarios.

Furthermore, our architecture enables variable parallelism on the level of input channels, output channels, kernel size, and batch size. This allows us to optimize the utilization of available hardware resources and thus increase efficiency and throughput.

\begin{comment}
\todo{start with motivation for memory reduction}

In the following, we describe the \ac{fpga} hardware architecture of our trainable \ac{cnn}, as depicted in Fig. \ref{fig:hardware_architecture},  where \ac{fp} is shown on the left and \ac{bp} on the right. As illustrated at the bottom, our implementation allows for training with either supervised \ac{mse} loss or with our novel unsupervised loss function.



\begin{figure}[!h]
	\centerline{\input{figures/tikz_hardware_architecture.tex}}
	\caption{Hardware architecture of trainable with kernel size $K$, padding $P$, stride $S$, dilation $D$ and number of channels $N_{ch}$. Arrows indicate streams of feature maps, either between subsequent layers or between \ac{fp} and \ac{bp}. Feature map buffers are shown in red.
 }
	\label{fig:hardware_architecture}
\end{figure}

%One major challenge of implementing a trainable \ac{cnn} for sequence detection on \ac{fpga} is the large amount of memory, required to store the feature maps of the \ac{fp} to be reused for the kernel's gradient calculation. For high sequence lengths, on-chip memory is not sufficient to store those feature maps, thus offloading to external DRAM is necessary, resulting in limited throughput. For instance, experiments showed that storing a sequence with the length of one Ethernet frame (\SI{1518}{byte}) requires four times as many \acp{bram} as utilized by the whole remaining architecture. Moreover, storing \num{5} Ethernet frames on-chip even exceeds the available \ac{bram} of a high-end \ac{fpga} like the \textit{Xilinx XCZU9EG\nobreakdash-2FFVB1156}.\\
%\todo{other solution: smaller sequence length -> more interruptions -> no stable communication}
To tackle this challenge, we take advantage of the sequential nature of convolution operations \eqref{eq_2} and \eqref{eq_3} in the \ac{bp}. The calculation of $\nabla i$ and $\nabla k$ can already start before all elements of $i$ and $\nabla o$ are available. Thus, we implement the \ac{fp} and \ac{bp} in a pipelined fashion, which allows processing \ac{fp} and \ac{bp} in parallel. Therefore the feature maps are read and written concurrently and the size of the buffers can be greatly reduced.
Moreover, we designed our layers in a way that \ac{fp} and \ac{bp} have similar latency. Therefore, the size of the feature map buffers is determined only by the depth of the pipeline and does not depend on the length of the sequence. This enables processing symbol-sequences of arbitrary length and thus increases flexibility.\\
To further boost the throughput and flexibility, our architecture allows for variable \ac{dop} on the level of input channels, output channels, and kernel size for \ac{fp} and \ac{bp}. Thereby, our architecture is suited for a wide range of communication scenarios from low-power to high-throughput. 


%Moreover, we tackle the challenge of different \ac{dop} for \ac{fp} and \ac{bp}. With a standard architecture different \acp{dop} would result in large buffer sizes as the feature maps are written faster by the \ac{fp} than they are read by the \ac{bp}. Therefore, the required buffer size would grow linear with increased sequence length resulting in a large memory demand for the large bit-sequences transmitted in communication systems. 
%We solve this problem by discarding a part of the feature map before buffering, so the \ac{bp} only operates on a subset of the data. This way, it is possible to balance the latency of \ac{fp} and \ac{bp}. Thereby, our architecture is suited for a wide range of communication scenarios from low-power to high-throughput. 
\end{comment}








==> chapters/related_work.tex <==
\section{Related Work}
\label{Sec:related_work}


Summarize related work about equalization for optcial channels (different ANN approaches? conventional methods -> Volterra)

Many different works regarding implementation and optimization of \acp{ann} for optical channel equalization on edge devices. 

% Experimental implementation of a neural network optical channel equalizer in restricted hardware using pruning and quantization 
\cite{ron2022} applied pruning and quantization to reduce the computational complexity  of the \ac{ann}  by up to \SI{78}{\percent} and the memory footprint by up to \SI{87}{\percent}. Therefore the performance of the equalizer is evaluated for different levels of sparsity with and without quantization applied. Afterwards a model with \SI{60}{\percent} sparsity is implemented on the Raspberry Pi 4 and on Nivida Jetson Nano. 

% Fixed-Point Analysis and FPGA Implementation of Deep Neural Network Based Equalizers for High-Speed PON
\cite{kaneda2021} implemented a \ac{ann} with two hidden layers on \ac{fpga} to evaluate various fixed-point quantization configurations. To increase the throughput they propose to use an \ac{ann} that outputs two symbols for joint classification. As a result, they show that a quantization of \num{4} bits per weight can be achieved without a significant drop in performance. 

% Towards FPGA Implementation of Neural Network-Based Nonlinearity Mitgation Equalizers in Coherent Optical Transmission Systems 
\cite{freire2022} evaluated the performance and complexity of \ac{ann}-based equalizers on \ac{fpga} and compared it to traditional digital backpropagation solutions. Therefore they design \ac{cnn} and \ac{bilstm}-based equalizers and implement them on \ac{fpga} using \ac{hls}. As a result, the \ac{bilstm} achieves higher communication performance than the traditional chromatic dispersion compensation block while requiring \num{2.5} times more \ac{fpga} resources.  

% Artificial Neural Network Nonlinear Equalizer for Coherent Optical OFDM
% \cite{jarajreh2015} 
% No FPGA implementation

% FPGA Implementation of Time-Interleaved Pruning Neural Network Equalizer for Short Reach Optical Interconnects
\cite{li2021} applied weight pruning techniques to a three-layer \ac{ann} to reduce the computational complexity and increase the number of channels processed in parallel. They report a \ac{fpga} resource reduction of \SI{55}{\percent} as compared to the dense network while maintaining the \ac{ber}. 





Summarize related work about ANN training (focus on low-power, sequence learning)

Most works implementing \acp{ann} on \ac{fpga} focus on the hardware implementation of the inference part only, while training the network on dedicated \acp{gpu} beforehand \addcitation. However, in recent years training on the \ac{fpga} itself using backpropagation became more popular to perform online fine-tuning on the edge \addcitation. 

% Towards efficient deep neural network training by FPGA-based batch-level parallelism (DarkFPGA)
In 2020 Luo et. al proposed an architecture for low-precision training of \acp{ann} on \acp{fpga} \cite{luo2020}. They explore parallelism on the level of batches with an optimised batch-oriented data pattern and tilling technique. The backpropagation is performed using \num{8}-bit integer weights to reduce complexity which allows for increased batch size and throughput. As a result the \ac{fpga}-based accelerator outperforms the \ac{cpu} in terms of throughput and the \ac{gpu} regarding energy consumption. 


% Automated CNN back-propagation pipeline generation for FPGA online training
\cite{mazouz2021} presented a framework to automatically generate an \ac{fpga} hardware design including backpropagation from the given \ac{cnn} model. A multi-objective optimization algorithm is used to explore the design space with respect to different levels of parallelism. They design a stream-based architecture using generic \acp{pe} to increase the hardware reuse between forward and backward pass. They report a speedup of the \ac{fpga} compared to \ac{cpu} and \ac{gpu} for a batch-size of one while the \ac{gpu} outperforms the \ac{fpga} for higher batch sizes. 

% FPGA Based Reconfigurable Coprocessor for Deep Convolutional Neural Network Training 
In \cite{clere2018} a \ac{ann} training accelerator is designed that can be reconfigured for different network structures by writing configuration parameters and input specifications to the \ac{bram}. The architecture consists of three different engines (forward propagation, gradient calculation, weight update) and is based on \num{18}-bit fixed-point representation. The design achieves a maximum throughput of \SI{280}{\giga\operations\per\second} on the HTC-K800 FPGA. 


As shown in this section, most \ac{fpga} \ac{ann} training implementations focus on maximizing the throughput while achieving higher energy efficiency than general purpose processors. 
However, the presented application -- which is mostly image classification --  does not rely on online training at the edge as training could  also be performed on high-performance server clusters without any power constraints. In contrast, our application requires low-latency retraining and therefore motivates for our novel low-latency streaming architecture. 

A similar scenario was presented in \cite{ney2022}, where a trainable demapper is implemented on \ac{fpga} to compensate for channel variations. However, in contrast to our work \cite{ney2022} relies on an oversimplified channel model, is based on fully-connected layers only, and does not provide a detailed quantization analysis.




\todo{Maybe no extra section for related work, but discuss in every subsection (NN FPGA equalizers: Intro), (FPGA training: hardware architecture), (automatic quantization: ANN Optimization) etc.}




==> figures/algo_training.tex <==
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\DontPrintSemicolon



\SetKwFor{For}{for (}{)}{}

%\algorithmstyle{ruled}
\begin{algorithm}
\normalsize 
\vspace*{0.1cm}
\label{Alg:training_flow}
\caption{Training flow of the \ac{gan}-equalizer}\label{alg:training}

\SetNoFillComment

$\Nti$: Number of \acsp*{ti}; \hspace{8pt}$N$: Number of symbols per \acs*{ti}\;
$\Nd$: Number of discriminator updates per \acs*{ti}\;
%$A(\bm{d})$: Function mapping the data to the symbols\;
%$M$: Order of the modulation format\;
%$\multiUniDis{a}{b}{N}$: $N$-dimensional uniform dist. of integers in range $[a, b]$ per dimension\;
$\multiNormDis{\mu}{\sigma^{2}}{N}$: $N$-dimensional normal distribution with each dimension's mean $\mu$ and variance $\sigma^{2}$\;
$\gamma_\text{ch}\mlr{\bm{x}}$: Function representing the channel distortions\;
$\varRefi$: Function returning the reference's variance at the \acs*{ti} $i$

\BlankLine
\For{$i=0$;\ $i<\Nti$;\ $i\text{++}$}{
	    \tcc{Train Discriminator}
	    \For{$j=0$;\ $j<\Nd$;\ $j\text{++}$}{
	    \tcc{Sample reference symbols}
	    %$ \bm{x}' = A(\bm{d}') + \multiNormDis{0}{\sigma_\mathrm{r}^{2}\mlr{i}}{N}$ with $\bm{d}'\sim \multiUniDis{1}{M}{N}$\;
	    $ \bm{x}' \sim P\mlr{\bm{x}} + \multiNormDis{0}{\varRefi}{N}$\;
	    \tcc{Sample channel output}
	    $ \bm{y} \sim \gamma_\text{ch}\mlr{\bm{x}} + \multiNormDis{0}{\varN}{N}$ with $\bm{x} \sim p\mlr{\bm{x}}$\;
	    \tcc{Generate fake symbols}
	    $\bm{z} = G(\bm{y})$\;
	    \tcc{Get predictions of D to calc loss}
	    $\text{loss}_\mathrm{D} = \text{BCE}(D(\bm{x}'), 1) + \text{BCE}(D(\bm{z}), 0) + \text{HWA}_\mathrm{D}$ \;
	    update parameters of $D$ based on $\text{loss}_\mathrm{D}$\;
    }
    \tcc{Train Generator}
    \tcc{Get prediction for $\bm{z}$ and calc loss}
    $\text{loss}_\mathrm{G} = \text{BCE}(D(\bm{z}), 1) + \text{HWA}_\mathrm{G}$\;
    update parameters of $G$ based on $\text{loss}_\mathrm{G}$\;
}
\end{algorithm}
